Search for supersymmetry in final states with charm jets and missing transverse momentum in 13 TeV $pp$ collisions with the ATLAS detector

A search for supersymmetric partners of top quarks decaying as $\tilde{t}_1\to c\tilde\chi^0_1$ and supersymmetric partners of charm quarks decaying as $\tilde{c}_1\to c\tilde\chi^0_1$, where $\tilde\chi^0_1$ is the lightest neutralino, is presented. The search uses 36.1 ${\rm fb}^{-1}$ $pp$ collision data at a centre-of-mass energy of 13 TeV collected by the ATLAS experiment at the Large Hadron Collider and is performed in final states with jets identified as containing charm hadrons. Assuming a 100% branching ratio to $c\tilde\chi^0_1$, top and charm squarks with masses up to 850 GeV are excluded at 95% confidence level for a massless lightest neutralino. For $m_{\tilde{t}_1,\tilde{c}_1}-m_{\tilde\chi^0_1} <$100 GeV, top and charm squark masses up to 500 GeV are excluded.

==> StopCharmRun2Paper-hepdata.tex <==
\section{HepData material}
%-------------------------------------------------------------------------------

This file is available for detailed tables etc.\ that are going to be
submitted to HepData or other similar destinations.

==> latex/sections/sryields.tex <==
           & SR1 & SR2 & SR3 & SR4 & SR5 & SR5T\\
Observed           & $59$ & $33$ & $23$ & $53$ & $68$ & $23$\\
%%
 bkg          & $60.58 \pm 11.15$ & $32.01 \pm 4.84$ & $30.66 \pm 5.76$ & $58.67 \pm 10.74$ & $71.52 \pm 10.05$ & $25.68 \pm 4.36$\\
%%
         $Z(\to\nu\nu)$+jets          & $37.09 \pm 7.75$ & $16.71 \pm 3.20$ & $17.33 \pm 4.74$ & $33.98 \pm 8.11$ & $50.98 \pm 8.44$ & $19.07 \pm 3.55$\\
%%
         Wtaunu\_ISR          & $6.62 \pm 3.11$ & $2.89 \pm 1.21$ & $5.38 \pm 1.57$ & $9.33 \pm 2.72$ & $8.15 \pm 1.91$ & $2.69 \pm 0.64$\\
%%
         Wtaunu\_TauFake          & $1.72 \pm 0.97$ & $1.76 \pm 0.85$ & $0.80 \pm 0.35$ & $0.52 \pm 0.24$ & $0.00 \pm 0.00$ & $0.01 \pm 0.00$\\
%%
         $t\bar{t}$          & $4.42 \pm 1.57$ & $5.49 \pm 2.57$ & $1.67_{-1.67}^{+2.06}$ & $2.61 \pm 1.68$ & $1.51_{-1.51}^{+1.76}$ & $0.17_{-0.17}^{+0.26}$\\
%%
         Zee          & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$\\
%%
         Zmumu          & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.04 \pm 0.01$ & $0.00 \pm 0.00$\\
%%
         Wmunu          & $2.08 \pm 0.97$ & $0.72 \pm 0.38$ & $1.16 \pm 0.32$ & $2.86 \pm 1.62$ & $2.91 \pm 0.80$ & $0.98 \pm 0.29$\\
%%
         Wenu          & $0.78 \pm 0.56$ & $1.10 \pm 0.52$ & $1.06 \pm 0.24$ & $1.99 \pm 0.54$ & $2.82 \pm 0.68$ & $0.86 \pm 0.22$\\
%%
         Single top          & $1.01_{-1.01}^{+1.04}$ & $0.11_{-0.11}^{+0.14}$ & $0.28_{-0.28}^{+0.31}$ & $0.49_{-0.49}^{+0.52}$ & $0.91_{-0.91}^{+1.02}$ & $0.18_{-0.18}^{+0.20}$\\
%%
         Diboson          & $6.28 \pm 2.09$ & $2.73 \pm 1.65$ & $2.43 \pm 0.74$ & $5.93 \pm 2.25$ & $3.95 \pm 1.10$ & $1.66 \pm 0.91$\\
%%
         Other          & $0.58 \pm 0.11$ & $0.49 \pm 0.11$ & $0.54 \pm 0.12$ & $0.96 \pm 0.21$ & $0.24 \pm 0.07$ & $0.05 \pm 0.01$\\
\hline\hline
Expected events before fit\\
\hline\hline

